M^3-Bench: Multi-Modal, Multi-Hop, Multi-Threaded Tool-Using MLLM Agent Benchmark

We present M^3-Bench, the first benchmark for evaluating multimodal tool use under the Model Context Protocol. The benchmark targets realistic, multi-hop and multi-threaded workflows that require visual grounding and textual reasoning, cross-tool dependencies, and persistence of intermediate resources across steps. We introduce a similarity-driven alignment that serializes each tool call, embeds signatures with a sentence encoder, and performs similarity-bucketed Hungarian matching to obtain auditable one-to-one correspondences. On top of this alignment, we report interpretable metrics that decouple semantic fidelity from workflow consistency. The benchmark spans 28 servers with 231 tools, and provides standardized trajectories curated through an Executor & Judge pipeline with human verification; an auxiliary four large language models (LLMs) judge ensemble reports end-task Task Completion and information grounding. Evaluations of representative state-of-the-art Multimodal LLMs (MLLMs) reveal persistent gaps in multimodal MCP tool use, particularly in argument fidelity and structure consistency, underscoring the need for methods that jointly reason over images, text, and tool graphs. Our Benchmark's anonymous repository is at https://github.com/EtaYang10th/Open-M3-Bench

==> trajectoryformat.tex <==
\makeatletter
% ──────────────────────────────────────────────────────────────────────────────
% Usage（用法速览，非功能代码）
%   \begin{twocolkv}{Title}
%     \KV{Key}{Value text ...}
%     \KV{Key2}{More text ...}
%     \KVsection{Section Title}   % 小节分隔（当前实现：对齐“第二列”）
%     \KVsplit                    % 虚线分隔
%     \KVcont{A continuation line without label ...}
%   \end{twocolkv}
%
% 你最常调的“参数旋钮”：
%   1) 线条粗细：   \kvRuleTop / \kvRuleMid / \kvRuleThin （单位 pt）
%   2) 虚线样式：   \kvDashLen（实段长度） / \kvDashGap（间隙）
%   3) 两栏占比：   \kv@labelwidth（左“标签列”宽度，常设为 \linewidth 的百分比）
%   4) 列间距：     \kv@labelsep（标签列与正文列的水平空隙）
%   5) 垂直空白：   list 的 \topsep / \itemsep / \parsep / \partopsep
%   6) 满宽横线横向外扩/回缩：见 \kv@fullrule 里对 \leftmargin 的偏移常数（16pt/-8pt）
%
% 版面/可分页性：
%   - 该设计基于 LaTeX 的 list 环境，天然可分页；与 longtable 无关。
%   - 横线通过 \rule() 画，宽度按“正文列 + 标签列”的总宽计算，并用 \leftmargin 做对齐校正。
%
% \KVsection 对齐说明（当前行为→“第二列”对齐）：
%   - 目前实现用 \item[] 开一个“空标签”的条目，因此标题从“正文列起始”（即第二列）对齐。
%   - 如果你想改成“第一列”（左边标签列）对齐，可将 \KVsection 的内部逻辑改为在行首用
%     \noindent 或 \hspace*{-\leftmargin} 做负缩进并重画横线。但本文件按你的要求未做任何改动。
% ──────────────────────────────────────────────────────────────────────────────

% ====== tunables（按需微调，近似 booktabs 的粗细）======
% 这些是全局“粗细/样式”旋钮，优先从这里调；单位 pt。
\newcommand\kvRuleTop{1pt}   % 顶/底横线厚度（≈ booktabs 的 \toprule/\bottomrule）
\newcommand\kvRuleMid{0.5pt}   % 中横线厚度（≈ \midrule；也用于小节下方线）
\newcommand\kvRuleThin{0.4pt}  % 虚线的线段粗细（不建议太细，0.2–0.4pt 区间较稳）
\newcommand\kvDashLen{5pt}     % 虚线“实段”的长度
\newcommand\kvDashGap{3pt}     % 虚线“空段”的长度

% ====== 内部：画“跨满标签列+正文列”的实线 ======
% 技术要点：
%   - list 环境中，正文起始会有 \leftmargin 的缩进；为了让横线“贯穿两列”并与外部版心对齐，
%     需要先向左回退（负 \leftmargin 的位移），再按“（正文宽 + 左缩进）”给出线长。
%   - 这里额外用了 +16pt / -8pt 的微调量，是经验性外观校正（例如避免线头/线尾被段前后 glue 吃掉，
%     或者与标题粗体字重叠造成的视觉短缺）。若你觉得略长/略短，可在此两处做对称性微调。
\newcommand{\kv@fullrule}[1]{%
    \noindent\hspace*{\dimexpr-\leftmargin+16pt\relax}% ← 往左拉回：覆盖标签列，并多拉 16pt
    \rule{\dimexpr\linewidth+\leftmargin-8pt\relax}{#1}\par% ← 线宽=正文宽+左缩进，再回收 8pt
}

% ====== 内部：画“跨满标签列+正文列”的虚线 ======
% 原理：用 \leaders + \hbox + \rule 生成连续的“实段/空段”循环，直至填满目标宽度。
% 宽度同样取“正文宽 + 左缩进”，以覆盖两列；这里没做 +16pt/-8pt 的额外校正（与上保持风格差异）。
\newcommand{\kv@fulldash}[3]{% #1=dashlen #2=gap #3=thickness
  \noindent\hspace*{-\leftmargin}% ← 回退左缩进，使虚线跨越两列
  \hbox to \dimexpr\linewidth+\leftmargin\relax{%
    \leaders\hbox{\rule{#1}{#3}\hskip #2}\hfill
  }\par
}

% ====== 公共别名：对齐 booktabs 语义 ======
% 这三条提供统一语义接口（上/中/下横线），便于全局换肤（仅改粗细变量即可）。
\newcommand{\KVtoprule}{\kv@fullrule{\kvRuleTop}}
\newcommand{\KVmidrule}{\kv@fullrule{\kvRuleMid}}
\newcommand{\KVbottomrule}{\kv@fullrule{\kvRuleTop}}
\newcommand{\KVdashline}{\kv@fulldash{\kvDashLen}{\kvDashGap}{\kvRuleThin}}

% ====== 环境：两栏友好、可分页的键值样式 ======
% 结构说明：
%   - 使用 list 做两列布局：左列为“标签”（\labelwidth），右列为“正文”，两列之间用 \labelsep 间隔。
%   - \kv@labelwidth / \kv@labelsep 是“主要外观”参数；一般只改这两个即可得到想要的占比/间距。
%   - 开头/结尾用 \KVtoprule/\KVbottomrule 包围，标题加粗放在两条顶线之间。
\newenvironment{twocolkv}[1]{%
  \begingroup
  \footnotesize                        % 全体字号（可改为 \small/\scriptsize 等）
  \setlength{\parindent}{0pt}%         % 段首不缩进
  \setlength{\parskip}{0pt}%           % 段间距为 0，避免键值间出现意外空白
  % 左标签列≈7%，右侧≈92%（可按需要改；两者之和不必正好=100%，因为还有 \labelsep）
  \def\kv@labelwidth{0.07\linewidth}%  % 左列宽度（相对 \linewidth 的比例）
  \def\kv@labelsep{0.6em}%             % 左右列的水平间距（过小会显挤，过大浪费空间）
    \KVtoprule                         % 顶部横线（1）
    \par\noindent\textbf{#1}\par        % 标题行（加粗）
    \vspace{-1pt}\KVtoprule              % 顶部横线（2）：形成“上下包围”的标题区域
  \begin{list}{}{%
    % 下面这些 list 参数共同决定“双栏版式”的几何关系：
    \setlength{\labelwidth}{\kv@labelwidth}% 左列宽度（用于放 \item[...] 的“标签”）
    \setlength{\leftmargin}{\kv@labelwidth}% 整体左缩进=左列宽度
    \addtolength{\leftmargin}{\kv@labelsep}% 再加上列间距 → 正文列起始位置
    \setlength{\labelsep}{\kv@labelsep}%   % 标签与正文之间的水平缝隙
    \setlength{\rightmargin}{0pt}%         % 右边不额外缩进（保持满宽）
    % 垂直节奏（可据版心紧凑度微调；统一在这里改）：
    \setlength{\topsep}{1pt}%              % 列表开始/结束与周围文本之间的垂直间距
    \setlength{\itemsep}{1pt}%             % 各 \item 之间的距离（键值行的行距感）
    \setlength{\parsep}{0pt}%              % 同一 \item 内多段文本之间的间距
    \setlength{\partopsep}{0pt}%           % 列表紧贴前段落时的额外间距（一般置 0）
  }%
}{%
  \end{list}%
  \KVbottomrule                          % 底部横线
  \endgroup
}

% 键值行（左列为粗体等宽体标签；右列为正文内容）
% - 你也可在调用时将 \texttt 替换为 \textsc 等（本定义保持与你原外观一致）。
\newcommand{\KV}[2]{\item[\textbf{\texttt{#1}}] #2}

% 小节标题（等价：上粗线 + 标题 + 中等粗线）
\newcommand{\KVsection}[1]{%
  \begingroup
  \renewcommand{\kv@fullrule}[1]{%
    \noindent\hspace*{-\leftmargin}% 左移回到第一列起点
    \rule{\dimexpr\linewidth+\leftmargin\relax}{##1}\par
  }%
  \KVmidrule
  \vspace{1pt}\noindent\hspace*{-\leftmargin}\textbf{#1}\par % 标题文字顶到第一列
  \vspace{-2pt}\KVmidrule
  \endgroup
}

% 分隔线（等价 \cdashline{1-2} 的视觉效果）：跨两列的虚线
\newcommand{\KVsplit}{\item[]\KVdashline}

% 无标签续行：在“第二列”（正文列）继续排一行，不占用标签列
\newcommand{\KVcont}[1]{\item[] #1}

\newenvironment{KVfinal}{%
  \par\begingroup
  \parindent=0pt \parskip=0pt
  % 让每个段落：左缩进 = -\leftmargin；行宽 = \linewidth+\leftmargin
  \parshape 1 -0\leftmargin \dimexpr\linewidth+\leftmargin\relax
}{%
  \par\endgroup
}

\makeatother

